Towards a Defense Against Federated Backdoor Attacks Under Continuous Training

Backdoor attacks are dangerous and difficult to prevent in federated learning (FL), where training data is sourced from untrusted clients over long periods of time. These difficulties arise because: (a) defenders in FL do not have access to raw training data, and (b) a new phenomenon we identify called backdoor leakage causes models trained continuously to eventually suffer from backdoors due to cumulative errors in defense mechanisms. We propose shadow learning, a framework for defending against backdoor attacks in the FL setting under long-range training. Shadow learning trains two models in parallel: a backbone model and a shadow model. The backbone is trained without any defense mechanism to obtain good performance on the main task. The shadow model combines filtering of malicious clients with early-stopping to control the attack success rate even as the data distribution changes. We theoretically motivate our design and show experimentally that our framework significantly improves upon existing defenses against backdoor attacks.

==> algorithm.tex <==
\section{Design}
\label{sec:design}

We propose a framework called \emph{shadow learning} 
% of training two models, a backbone  and a shadow model, in parallel 
% (Algorithm~\ref{alg:framework}, App. 
% \ref{sce:alg}), 
that builds upon three  main insights. 
% We propose a novel framework of training two models, a backbone  and a shadow model, in parallel 
% (Algorithm~\ref{alg:framework}),  
% motivated by a failure mode of existing defense algorithms: backdoor leakage (\S\ref{sec:backdoor-leakage}). 
% We build upon two main techniques:  early-stopping (\S\ref{sec:early-stopping}) and robust covariance estimation (\S\ref{sec:robust}). 

% \subsection{Backdoor leakage}
% \label{sec:backdoor-leakage}

\paragraph{Insight 1: Every existing approach suffers from backdoor leakage.}
\label{sec:backdoor-leakage}
Most backdoor defenses significantly reduce the effect of backdoor attacks in a single round. 
However, a small fraction of malicious gradients or model updates always go undetected. 
Over many training rounds (which are required under distribution drift, for instance), this {\em backdoor leakage} eventually leads to a fully-backdoored model. 
Figure \ref{fig:backdoor_leakage} shows the ASR over the training rounds of a backdoored classifier on the EMNIST dataset of handwritten digits. 
We compare against baselines including SPECTRE \cite{spectre} (both gradient-based G-SPECTRE and representation-based R-SPECTRE), RFA \cite{geomedian}, Multi-Krum \cite{krum},  norm clipping and/or noise addition \cite{backdoor}, 
 CRFL \cite{crfl}, FLAME \cite{flame},  and FoolsGold \cite{foolsgold}. 
Experimental details are explained %in detail
in Appendix~\ref{sec:compete}.
%, and \S\ref{sec:robust} for R-SPECTRE and G-SPECTRE.
%To show the backdoor leakage phenomenon in Fig. \ref{fig:backdoor_leakage},
For a relatively small $\alpha=3\%$ and for $12,000$ rounds, 
we observe the attack success rate (ASR) of all competing  defenses eventually approach one.
% \gf{Move this sentence elsewhere?
% To overcome backdoor leakage, we introduce Algorithm~\ref{alg:framework}, which  consistently achieves small ASR throughout the training.}
%Among all baselines, the representation-based SPECTRE has the slowest backdoor learning rate, and takes around $10000$ rounds to converge on ASR.
% On the other hand,  Algorithm~\ref{alg:framework} achieves an ASR of $0.0013$ for EMNIST and $0.0092$ for CIFAR-10.
%The early stopped shadow network when the training accuracy on benign samples with the target label converges, ASR is independent of the training round.  %, indicating the success of the defense.
These experiments are under the static setting where  data distribution is fixed over time; we show results in dynamic settings in \S\ref{section:time_varying}. 
The main takeaway is that \textbf{in the continual FL setting, we cannot use the predictions of a single backdoor-resistant model that is trained for too long.}






\paragraph{Insight 2: Early-stopping helps when $\alpha$ is small.}
%Although backdoor leakage eventually causes prior defenses to fail, we see in Figure \ref{fig:backdoor_leakage} that certain defenses (e.g., R-SPECTRE) can substantially slow down the rate at which backdoor attacks are learned. 
%This suggests a natural defense: can we couple an existing defense with early-stopping 
Backdoor leakage suggests a natural defense: can we adopt early-stopping to ensure that the model does not have enough time to learn a backdoor? 
The answer depends on the relative difficulty of the main task compared to the backdoor task, as well as the adversarial fraction $\alpha$. 
For example, Figure \ref{fig:earlystop} shows that on EMNIST (same setting as Figure \ref{fig:backdoor_leakage}), when $\alpha = 3\%$, the backdoor is learned more slowly than the main task: 
%For $\alpha = 3\%$, 
the main task reaches an accuracy of $0.99$, while the attack success rate %backdoor 
is no more than $0.01$.
This suggests that early-stopping can be effective. 
On the other hand, Li \emph{et al.} \cite{li2021anti} found that backdoors are learned \emph{faster} than the main task, and propose a defense based on this observation. 
% Our experiments suggest that their observation is only true for large $\alpha$.
Indeed, Figure \ref{fig:earlystop} shows that when $\alpha = 25\%$, the previous trend is reversed: the backdoor is learned faster than the main task.
Over many experiments on multiple datasets, we observe that \textbf{early-stopping is only an effective defense when $\alpha$ is small enough relative to the main task difficulty.}
% We make this intuition precise in \S\ref{sec:analysis}.

\paragraph{Insight 3: We can reduce $\alpha$ with robust filtering} 
\label{sec:robust} 

Since early-stopping helps when $\alpha$ is small, we can use FL-compatible filtering techniques to reduce the effective $\alpha$ at any round. 
Filtering algorithms are designed to separate malicious data from benign data, and they often use techniques from robust statistics and outlier detection. 
Many proposed defenses can be viewed as filtering algorithms, including (Multi-)Krum,  activation clustering , and SPECTRE  (more complete list in Appendix \ref{app:related}).
Any of these can be adapted to the FL setting to reduce the effective $\alpha$.
% to filter out malicious client updates. 
% This makes early stopping more effective. 
% Specifically, we use SPECTRE for outlier detection based on robust covariance estimation \cite{spectre}.
% SPECTRE has been shown to be effective in identifying backdoored attack samples in the non-FL setting. %(Appendix~\ref{sec:compete}). 
% A straightforward adaptation is what we call R-SPECTRE: this applies SPECTRE to identify corrupt clients at every round in the FL setting, and uses only  model updates from clients that are identified as benign. 
% Figure~\ref{fig:backdoor_leakage} shows that R-SPECTRE is significantly more effective than other defenses, as shown by the relatively slow increase in the ASR (though it eventually suffers from backdoor leakage). We use SPECTRE to filter out malicious clients and reduce our effective $\alpha$, then train an early-stopped model with SPECTRE-filtered model updates. 
% % \gf{Move this sentence elsewhere?
% Using this intuition, we next introduce Algorithm~\ref{alg:framework}, which  consistently achieves small ASR throughout training.


\subsection{Shadow Learning: A Defense Framework}
\label{sec:algo}

For simplicity, we first explain the framework assuming that the defender knows the target class $\ell$; we then explain how to relax this assumption (pseudocode in Algorithm \ref{alg:framework_extend}). 

\paragraph{Training.}
 Shadow learning combines the prior insights by training two models: the \emph{backbone model} and the \emph{shadow model} (Framework~\ref{alg:early}). 
The backbone model is trained to be {\em backdoored} but stable (i.e., insensitive to  distribution shifts and  filtering by our algorithm). 
In training, it is updated in each round using all (including malicious) client data. 
At test time, we only use it if the prediction is \emph{not} the target label. 
Otherwise, we resort to the shadow model,
% trained as follows. 
% Once we have learned a good filter parametrized by $(\hat {\boldsymbol \Sigma},\hat{\boldsymbol \mu},T,{\boldsymbol U})$, 
% a shadow model 
which is trained on filtered data that removes suspected malicious clients at each round.
This filtering reduces the effective $\alpha$ for the shadow model. 
Finally, the shadow model is early-stopped to avoid backdoor leakage.

% The main innovations are $(i)$ we use the backbone model to learn the parameters of a {\sc Filter} (Algorithm~\ref{alg:filter} in Appendix~\ref{sce:alg}) that can filter out most of the poisoned model updates, and $(ii)$ we use {\sc Filter} to reduce the fraction of poisoned model updates and train another network, shadow model, 
% but with {\em early stopping}. 
% The G-SPECTRE and R-SPECTRE curves in Figure~\ref{fig:backdoor_leakage} shows that 
% if we train a single model that is trained only on filtered model updates in each round, backdoor leakage eventually allows the backdoor to emerge. 
% Instead, under our framework, 
In more detail,
the \emph{backbone model} $\backbone$ is trained continually on all available client data, and thus is backdoored (see Figure \ref{fig:shadow-training}). However, it still serves two purposes: $(i)$ it is used to predict the non-target classes (since it has seen all the past training data and hence is resilient to changing datasets), and $(ii)$ it is used to learn parameters of a filter that can filter out poisoned model updates. 
Concretely, in each training round $r$, the backbone model $\backbone$ is updated on client data from all the clients in the  set $\clientset_{r}$ (line~\ref{line:backbone} Alg.~\ref{alg:framework}). 
% which is renewed once the data distribution of sample with target label $\targetlabel$ changes.
% In our implementation, this condition is determined by whether the

%These models are updated every $R$ rounds in what we call a \emph{retraining period}. 
%In practice, $R\geq 1$ should be chosen based on computational constraints; the shorter the retraining period, the better our backdoor performance metrics, but each retraining period incurs additional computational overhead.

% updated normally (i.e., according to whatever federated optimization algorithm is being used).
% The main added complexity of our algorithm is that we also train a shadow model $\shadow$ as follows. 
In parallel, we train the \emph{shadow model} $\shadow$ on filtered model updates and also early stopped such that it can robustly make predictions for the target label. As it is early stopped, we need to retrain the model periodically from a random initialization in every \emph{retraining period} to handle changing data distributions. A retraining period starts every time the target label distribution changes; in practice, we choose rounds where the training accuracy of the backbone model $\backbone$ on samples with the target label $\targetlabel$ changes by more than a threshold $\epsilon_1$ (lines \ref{line:renew1}-\ref{line:renew2}). 
%We assume we know the target label $\ell$, since there are target label detectors that have shown empirical successes, e.g., \cite[Algorithm 4]{spectre}. 
At the start of each retraining period, the server randomly initializes a new shadow model  $\shadow$ of the same architecture as $\backbone$. 
We say  $\backbone$ has converged on $\targetlabel$ if the difference between the training accuracy on samples with label $\targetlabel$ between two consecutive rounds is smaller than a convergence threshold $\epsilon_2$. 
The next time backbone $\backbone$ converges on the target label $\targetlabel$ distribution (call it round $r_0$, line \ref{line:converge}), we commence training $\shadow$ on filtered client sets $\{\mathcal{C}'_{r}\}_{r\geq r_0}$ until it is early-stopped. 
% \gf{REMOVE? We analyze a canonical example in \S\ref{sec:analysis} and show that $(i)$ the filtering we propose successfully learns a poison detector under certain separation conditions (Theorem~\ref{thm:main}), and $(ii)$ once filtering sufficiently reduces the fraction of poisoned model updates, early stopping learns a clean model  (Corollary~\ref{coro:early}).}


\begin{figure}
\centering
%\subfigure[Example of training dynamics of the backbone model $\backbone$ and shadow model $\shadow$ \gf{Move this plot later to \S\ref{sec:algo} and replace with early stopping figure}]
\vspace{-0.3cm}
\includegraphics[width=\linewidth]{img/015_illustrate.pdf}
\caption{Example of training dynamics of the backbone model $\backbone$ and shadow model $\shadow$}
\label{fig:shadow-training}
\vspace{-0.2cm}
\end{figure}


% Suppose a retraining period starts at round $r_0$.
Concretely, consider retraining a shadow model from round $r_0$ (e.g., in Figure \ref{fig:shadow-training}, $r_0=600$).
In each round $r \geq r_0$, we recompute the filtered client set $\mathcal{C}_{r}'$ whose data is used to train the shadow model $\shadow$. 
% for training the shadow model $\shadow$, 
% For every round $r$ of the retraining period, 
This is done by first having each client $c\in \clientset_{r}$ locally average the representations\footnote{E.g., these can be taken from the penultimate layer of $\backbone$.} of samples in $\database_c$ with target label $\targetlabel$; this average is sent to the server for filtering. 
To get the filter, in the first collection round (i.e., $r=600$), the server calls {\sc GetThreshold}, which returns filter parameters $\boldsymbol \theta$ and a threshold $T$; these are used in {\sc Filter} (Alg. \ref{alg:filter}) to remove malicious clients. 

Although our framework supports any filtering algorithm, we empirically find SPECTRE \cite{spectre} to be an effective filtering algorithm (e.g., it has the slowest backdoor leakage in Fig. \ref{fig:backdoor_leakage}) and use it for the remainder of this work. If the filtering algorithm is SPECTRE, {\sc GetThreshold} returns the parameters $\boldsymbol \theta = (\hat {\boldsymbol \Sigma},\hat{\boldsymbol \mu},T,{\boldsymbol U})$ for the robust covariance $\hat{ \boldsymbol  \Sigma}$, 
robust mean $\hat{\boldsymbol \mu}$, filtering threshold $T$, and an orthonormal matrix $U$ representing the top $k$ PCA vectors for the representations $\{{\boldsymbol h}_j\in{\mathbb R}^d\}_{j\in\mathcal{C}_{r}}$. 
% Specifically, in (lines \ref{line:threshold1}-\ref{line:threshold2}), we call {\sc GetThreshold} that $(i)$ finds top $k$ PCA directions represented by an orthonormal matrix ${\boldsymbol U}\in{\mathbb R}^{d\times k}$ for the representations $\{{\boldsymbol h}_j\in{\mathbb R}^d\}_{j\in\mathcal{C}_{r}}$, $(ii)$  runs a robust covariance estimator from \cite{diakonikolas2017being} to estimate the covariance $\boldsymbol{\Sigma}$ and mean $\boldsymbol{\mu}$ of the benign representations using the combined benign and corrupted representations (which is critical in achieving a good filter as demonstrated in \cite{spectre}), and $(iii)$ calculates an outlier score called {\em the QUantum Entropy (QUE) score} of all representations with a QUE parameter $\beta$ to find the threshold $T$ for outlier detection.
The filtering threshold $T$ is set in this case as the $1.5\bar{\alpha}|\mathcal{C}|$-th largest QUE score, which intuitively captures how ``abnormal" a sample is (Alg. \ref{alg:que}), where $\bar{\alpha}$ is an estimated upper bound on the malicious rate.
The SPECTRE filtering process is detailed in Algorithms \ref{alg:threshold} and \ref{alg:filter} (Appendix \ref{sce:alg}).
%, and the top $k$ left singular vectors of the centered representations is stored as $\boldsymbol{U}$ (lines 15-18). 


% The main idea of our approach is that the backbone network is trained to be {\em backdoored} and is stable (insensitive to the changes due to client distribution shifts and how we filter data). At test time, we only use it if the prediction is not the target label. Otherwise we resort to the shadow model trained as follows. 
% Once we have learned a good filter parametrized by $(\hat {\boldsymbol \Sigma},\hat{\boldsymbol \mu},T,{\boldsymbol U})$, 
% a shadow model is trained on  filtered data that filters out suspected clients at each subsequent round until it is early-stopped.
%a new filter is learned or the shadow networks re-initialized to random weights.
% In the client filtering process, the collected representations are projected down to a $k$-dimensional space by $\boldsymbol{U}$, then whitened to get $\tilde {\boldsymbol{h}}_j = \boldsymbol{\hat\Sigma}^{-1/2} (\boldsymbol{U}^T\boldsymbol{h}_j- \boldsymbol{\hat\mu} ) \in{\mathbb R}^k$ for all $j\in \mathcal{C}_{r}$. The projection onto ${\boldsymbol U}$ is to reduce computational complexity, which is less critical for performance of the filter. The whitening with clean covariance $\boldsymbol{\hat\Sigma}$ and clean mean  $\boldsymbol{\hat\mu}$ ensures that the poisoned representations stand out from the clean ones and is critical for the performance of the filter. 
% Based on the whitened representations, the server calculates QUE scores (which roughly translates as the scaled-norm of the whitened representation) for all clients and keeps the clients with scores less than the threshold $T$ as $\mathcal{C}'_{r}$ ({\sc Filter} in line \ref{line:filter}).
% The details of {\sc GetThreshold} and the client filtering process, {\sc Filter}, are shown in Algorithms \ref{alg:threshold} and \ref{alg:filter}.



%After $\backbone$ being converged on label $\targetlabel$, $\shadow$ is trained by the filtered client set $\mathcal{C}'$ until it is early-stopped. To obtain $\mathcal{C}'$, the serve also collects the averaged representations of samples with label $L$. Multiplied by $\boldsymbol{U}^{\top}$, the representations are reduced to $k$ dimensions, and then they are whitened by $\boldsymbol{\Sigma}$ and $\boldsymbol{\mu}$. After calculating the QUE scores, the server keeps the users with scores smaller than the threshold $T$ as $\mathcal{C}'$.

The shadow network $\shadow$ is early-stopped once the training accuracy on benign target samples converges. To determine the early-stopping point,  clients send the training accuracy on samples with label $\targetlabel$ to the server. If the difference between the average values of the largest $(1-\bar{\alpha})$-fraction training accuracy in two consecutive rounds is smaller than  $\epsilon_2$, $\shadow$ is early-stopped.

We illustrate the training process of the backbone model $\backbone$ and shadow model $\shadow$ in one retraining period with malicious rate $\alpha = 0.15$ under CIFAR-10  in Figure \ref{fig:shadow-training}.
Once the backbone model $\backbone$ converges on the target label $\targetlabel$ (illustrated by the blue dotted line), the server starts training the shadow model $\shadow$ based on the filtered client set. $\shadow$ is early-stopped once its training accuracy on benign target samples converges (illustrated by the orange dotted line).

\paragraph{Testing.}
At test time, all unlabeled samples are first passed through backbone $\backbone$. If predicted as the target label $\targetlabel$, the sample is passed through the early-stopped shadow network $\shadow$, whose prediction is taken as the final output. 


%We also illustrate the learning rate of the backdoor samples and benign samples with the target label $\targetlabel$ in backbone and shadow networks in Fig.\ref{fig:learning_rate}.
%We can observe that with malicious rate $\alpha = 0.15\%$, the backdoor learning rate in the backbone network is faster than the learning rate of benign target samples.
%However, after the filtering process, the backdoor learning rate becomes much more slower in the shadow network due to the significant reduction of malicious rate in the filtered client set. 
%The drop of the backdoor learning rate ensures the success of our algorithm on defending against backdoor attacks  with large malicious rate. 

%\begin{figure}[htbp]
%\centering
%\includegraphics[width=0.46\linewidth]{img/015_illustrate.pdf}
%\caption{Training Process of the Backbone Model $\backbone$ and Shadow Model $\shadow$}
%\label{fig:learning_rate}
%\end{figure}


% The overall algorithm is shown as follows.


 
% \begin{algorithm}[htpb]
%     \label{alg:early}
%     \LinesNumbered
% 	\BlankLine
% 	\SetKwInOut{Input}{input}
% 	\SetKwInOut{Output}{output}
% 	\caption{Shadow learning framework}
% 	\label{alg:framework}
% 	\Input{malicious rate upper bound $\bar{\alpha}$, target label $\targetlabel$,
% 	retraining threshold $\epsilon_1$, convergence threshold $\epsilon_2$, dimension $k$, QUE parameter $\beta$.}
% 	\BlankLine
% 	Initialize the networks $\backbone$, $\shadow$; \  $converge \leftarrow \text{False}$; \  $filter\_learned \leftarrow \text{False}$\;
% 	\For{\text{each training round} $r$}{
% 	Train the backbone network $\backbone$ with client set $\mathcal{C}_r$\label{line:backbone}\;
% 	The server collects training accuracy on samples with label $\targetlabel$ of each client in $\mathcal{C}_r$, and calculates the mean value $A_N^{(r)}$\;
% 	%Each client $j$ in $\mathcal{C}_i$ uploads the training accuracy $A_j^{(i)}$ of samples with label $L$\;
% 	\If{$converge$  \ {\rm {and}} \ $\left|A_N^{(r)}-A_{N}^{(r-1)}\right|>\epsilon_1$ \label{line:renew1}}{ 
% 	    $converge \leftarrow \text{False}$; \ 
% 	    $filter\_learned \leftarrow \text{False}$\;
% 	    Initialize the shadow network $\shadow$\label{line:renew2}\;
% 	}
% 	{\bf if} {\em not} $converge$ \ {\rm {and}} \ $\left|A_N^{(r)}-A_{N}^{(r-1)}\right|<\epsilon_2$
% 	 {\bf \ then } $converge \leftarrow \text{True}$ \label{line:converge}\; 
% 	%\If{ not $converge$ \ {\rm {and}} \ $\left|A_N^{(r)}-A_{N}^{(r-1)}\right|<\epsilon_2$\label{line:converge1}}{ %\ for at least $1-\alpha$ portion of clients}{ $converge \leftarrow \text{True}$ \label{line:converge2}\; }
% 	\If{$converge$}{
% 		Each client $j$ in $\mathcal{C}_r$ uploads the averaged representation $\boldsymbol{h}_j^{(r)}$ of samples with label $\targetlabel$\;
% 		\If{not $filter\_learned$\label{line:threshold1}}{
% 			$\boldsymbol{\hat\Sigma}, \boldsymbol{\hat\mu}, T, \boldsymbol{U} \leftarrow \text{{\sc GetThreshold}}\left(\left\{\boldsymbol{h}_j^{(r)}\right\}_{j\in \mathcal{C}_r}, \bar{\alpha}, k, \beta \right)$ {\hfill [Algorithm \ref{alg:threshold}]}
			
% 			$filter\_learned \leftarrow \text{True}$; \ 
% 			$early\_stop \leftarrow \text{False}$\label{line:threshold2}\;
% 			}
% 		\If{not $early\_stop$}{
% 			$\mathcal{C}'_r\leftarrow \text{{\sc Filter}}\left(\left\{\boldsymbol{U}^{\top}\boldsymbol{h}_j^{(r)}\right\}_{j\in \mathcal{C}_r}, \boldsymbol{\hat\Sigma}, \boldsymbol{\hat\mu}, T, \beta \right)$ 
% 			\label{line:filter}
% 			{\hfill [Algorithm \ref{alg:filter}]}
			
% 			Train $\shadow$ with client set $\mathcal{C}'_r$\;
% 			The server collects training accuracy on samples with label $\targetlabel$ of each client in $\mathcal{C}'_r$, and calculates the mean of the largest $(1-\bar{\alpha})$-fraction values as $A_{N'}^{(r)}$\;
% 			%Each client $j$ in $\mathcal{C}'$ uploads the training accuracy $B_j^{(i)}$ of samples with label $L$\;
% 			{\bf if } 
% 			$\left|A_{N'}^{(r)}-A_{N'}^{(r-1)}\right|<\epsilon_2$ {\bf \  then } 
% 				$early\_stop \leftarrow \text{True}$.
			
% 			%\If{$\left|A_{N'}^{(r)}-A_{N'}^{(r-1)}\right|<\epsilon_2$}{ %\ for at least $1-\alpha$ portion of clients}{
% 			%	$early\_stop \leftarrow \text{True}$.
% 			%	}
% 			}
% 		}
% 	}
% \end{algorithm}
\begin{algorithm}[htbp] %[htbp]
    \label{alg:early}
    \LinesNumbered
	\BlankLine
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	\caption{Shadow learning framework}
	\label{alg:framework}
	\Input{malicious rate upper bound $\bar{\alpha}$, target label $\targetlabel$,
	retraining threshold $\epsilon_1$, convergence threshold $\epsilon_2$, dimension $k$, filtering hyperparameters $\boldsymbol \beta$.}
	\BlankLine
	Initialize the networks $\backbone$, $\shadow$; \  $converge \leftarrow \text{False}$; \  $filter\_learned \leftarrow \text{False}$\;
	\For{\text{each training round} $r$}{
	Train the backbone network $\backbone$ with client set $\mathcal{C}_r$\label{line:backbone}\;
	The server collects training accuracy on samples with label $\targetlabel$ of each client in $\mathcal{C}_r$, and calculates the mean value $A_N^{(r)}$\;
	%Each client $j$ in $\mathcal{C}_i$ uploads the training accuracy $A_j^{(i)}$ of samples with label $L$\;
	\If{$converge$  \ {\rm {and}} \ $\left|A_N^{(r)}-A_{N}^{(r-1)}\right|>\epsilon_1$ \label{line:renew1}}{ 
	    $converge \leftarrow \text{False}$; \ 
	    $filter\_learned \leftarrow \text{False}$\;
	    Initialize the shadow network $\shadow$\label{line:renew2}\;
	}
	{\bf if} {\em not} $converge$ \ {\rm {and}} \ $\left|A_N^{(r)}-A_{N}^{(r-1)}\right|<\epsilon_2$
	 {\bf \ then } $converge \leftarrow \text{True}$ \label{line:converge}\; 
	%\If{ not $converge$ \ {\rm {and}} \ $\left|A_N^{(r)}-A_{N}^{(r-1)}\right|<\epsilon_2$\label{line:converge1}}{ %\ for at least $1-\alpha$ portion of clients}{ $converge \leftarrow \text{True}$ \label{line:converge2}\; }
	\If{$converge$}{
		Each client $j$ in $\mathcal{C}_r$ uploads the averaged representation $\boldsymbol{h}_j^{(r)}$ of samples with label $\targetlabel$\;
		\If{not $filter\_learned$\label{line:threshold1}}{
			$\boldsymbol{\theta}, T \leftarrow \text{{\sc GetThreshold}}\left(\left\{\boldsymbol{h}_j^{(r)}\right\}_{j\in \mathcal{C}_r}, \bar{\alpha}, k, \boldsymbol \beta \right)$ {\hfill [Algorithm \ref{alg:threshold}]}
			
			$filter\_learned \leftarrow \text{True}$; \ 
			$early\_stop \leftarrow \text{False}$\label{line:threshold2}\;
			}
		\If{not $early\_stop$}{
			$\mathcal{C}'_r\leftarrow \text{{\sc Filter}}\left(\left\{\boldsymbol{h}_j^{(r)}\right\}_{j\in \mathcal{C}_r}, \boldsymbol{\theta}, T, \boldsymbol \beta \right)$ 
			\label{line:filter}
			{\hfill [Algorithm \ref{alg:filter}]}
			
			Train $\shadow$ with client set $\mathcal{C}'_r$\;
			The server collects training accuracy on samples with label $\targetlabel$ of each client in $\mathcal{C}'_r$, and calculates the mean of the largest $(1-\bar{\alpha})$-fraction values as $A_{N'}^{(r)}$\;
			%Each client $j$ in $\mathcal{C}'$ uploads the training accuracy $B_j^{(i)}$ of samples with label $L$\;
			{\bf if } 
			$\left|A_{N'}^{(r)}-A_{N'}^{(r-1)}\right|<\epsilon_2$ {\bf \  then } 
				$early\_stop \leftarrow \text{True}$.
			
			%\If{$\left|A_{N'}^{(r)}-A_{N'}^{(r-1)}\right|<\epsilon_2$}{ %\ for at least $1-\alpha$ portion of clients}{
			%	$early\_stop \leftarrow \text{True}$.
			%	}
			}
		}
	}
\end{algorithm}
% \vspace{-5mm}

% In Algorithm \ref{alg:framework}, line 5-7 renews a retraining period once the data distribution of the samples with the target label $\targetlabel$ changes, and line 8-9 determines whether the backbone network $\backbone$ converges on label $\targetlabel$. In each retraining period, we conduct robust estimation and calculate QUE score threshold based on SPECTRE once $\backbone$ converges on label $\targetlabel$ in line 12-14. The shadow network $\shadow$ is then trained based on the filtered client set until it is early-stopped in line 15-18.
% Line 19-20 determines whether $\shadow$ should be early-stopped. The details of line 13 and the client filtering process in line 16 are shown in Algorithm \ref{alg:threshold} and \ref{alg:filter}.


\paragraph{Unknown target label $\ell$.}
% In practice, the adversary may have only partial (or no) knowledge of the target label $\ell$.
% Even in these cases, shadow learning can make meaningful progress. 
Suppose that instead of knowing $\ell$ exactly, the defender knows it to be in some set $S_\ell\subseteq [L]$. 
In this case, our framework generalizes by learning a different shadow network $N'_{y}$ and filter for each label $y \in S_\ell$.
It then chooses a set of labels $S_\ell' \subseteq S_\ell$ whose filters have the greatest separation between estimated benign and malicious clients. 
% This process will be specific to the filtering algorithm; 
For instance, under SPECTRE, this is done by comparing QUE scores for estimated outliers compared to inliers for each label (Alg. \ref{alg:framework_extend}, App. \ref{algorithm_extended}).
At test time, samples are first passed through the backbone $\backbone$. If the label prediction $y$ is in the filtered target set $S'_{\targetlabel}$, the sample is passed through the early-stopped shadow network $\shadow_y$, whose prediction is taken as the final output. 
















==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{app:ethical} of the Appendix.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section \ref{app:ethical} of the Appendix.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section \ref{sec:analysis} of the main body and Section \ref{Sec:proof} of the Appendix.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{Section \ref{Sec:proof} of the Appendix contains all proofs.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{All experimental details are in Section \ref{sec:experiments} of the main body and Section \ref{sec:compete} of the Appendix.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
        \answerYes{These are reported in Section \ref{sec:additional_exp} of the Appendix.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{These are reported in Section \ref{cost} of the Appendix.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section \ref{sec:experiments} of the main body and Section \ref{sec:compete} of the Appendix.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See the supplementary material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> experiment.tex <==
\section{Experimental results}
\label{sec:experiments}
%To demonstrate the value of our framework, we train backdoored classifiers on the EMNIST \cite{emnist} and CIFAR-10 \cite{cifar10} datasets.
%We compare with  state-of-the-art defense algorithms under the federated setting: SPECTRE (\cite{spectre}, both gradient- and representation-based), Robust Federated Aggregation (RFA) (\cite{geomedian}), Norm Clipping, and Noise Adding (\cite{backdoor}). 

We evaluate shadow learning (with R-SPECTRE filtering) on 4 datasets: EMNIST \cite{emnist}, CIFAR-10, %\cite{cifar10}, 
CIFAR-100 \cite{cifar10}, and Tiny ImageNet \cite{le2015tiny} datasets.
We compare with 8 state-of-the-art defense algorithms under the federated setting: 
 SPECTRE (gradient- and representation-based))\cite{spectre}, Robust Federated Aggregation (RFA) \cite{geomedian}, Norm Clipping, Noise Adding \cite{backdoor}, CRFL \cite{crfl}, FLAME \cite{flame}, Multi-Krum \cite{krum} and FoolsGold \cite{foolsgold}.
We give a detailed explanation of each in Appendix~\ref{sec:compete}, with hyperparameter settings. 

We consider a worst-case adversary that corrupts a full $\alpha$ fraction of clients in each round. In Appendix \ref{app:adaptive_alpha}, we study a relaxed threat model where the adversary can adapt their corrupt client fraction $\alpha(t)$ over time to take advantage of shadow model learning. 
% Norm Clipping bounds the norm of each model update to a threshold $M$, and Noise Adding adds Gaussian noise to the model updates. 
% In our experiments, we set the norm threshold $M=3$ and added zero-mean independent Gaussian noise with variance $\sigma^2 = 0.03$ to each coordinate.
% We implement RFA with 4-iteration Weiszfeld’s Algorithm.
% In all experiments, we set the malicious rate $\alpha$ as its upper bound, i.e., $\alpha = \bar{\alpha}$, let the dimensionality reduction parameter $k$ be $32$ and set the QUE parameter $\beta$ as $4$ in Algorithm~\ref{alg:framework}. We set the retraining threshold $\epsilon_1$ as $2\%$, and the convergence threshold $\epsilon_2$ as $0.05\%$.
% %We also show the backdoor leakage problem in all baseline algorithms, and conduct ablation study to show that each component of our algorithm is necessary for backdoor attack defense. 


%\medskip\noindent{\bf Baselines.}
%We compare our defense algorithm with SPECTRE (\cite{spectre}), Robust Federated Aggregation (RFA) (\cite{geomedian}), Norm Clipping and Noise Adding (\cite{backdoor}).

% SPECTRE adopts robust covariance estimation and data whitening to amplify the spectral signature of corrupted data, and then detect backdoor samples based on quantum entropy score.
% In federated learning settings, we adopt gradient-based and representation-based SPECTRE, which takes as input the gradient updates or representations of local training samples from the clients respectively.
% For both versions, we conduct the robust estimation and quantum score filtering every training round regardless of the computation constraints.

% RFA provides a robust secure aggregation oracle based on the geometric median, which is calculated by the Weiszfeld’s Algorithm. In our experiments, we implement RFA with 4-iteration Weiszfeld’s Algorithm.

% Norm Clipping defense bounds the norm of each model update to at most some threshold $M$, and Noise Adding method is to add a small amount of Gaussian noise to the updates. In our experiments, we set the norm threshold $M$ as $3$ and add independent Gaussian noise with variance $0.03$ to each coordinate.

% \medskip\noindent{\bf Experimental Setup.}
% \label{sec:experimental-setup}
 %of writer-annotated handwritten digits, where 
% As for the EMNIST dataset, there are 3383 users with roughly 100 images in ten labels per user with heterogeneous label distributions. We train a
% convolutional network with two convolutional layers, max-pooling, dropout, and two dense layers. %as in the Federated Learning task suite from (\cite{reddi2020}).
% CIFAR-10 dataset has $50,000$ training examples, with $5000$ samples in each label. We  partition those samples to $500$ users uniformly at random and  train a ResNet-18 \cite{he2016deep}.

% For both datasets, the server randomly selects $50$ clients each round, and each client trains the current model with the local data with batch size $20$,  learning rate $0.1$, and for two iterations. The server learning rate is $0.5$.  
% The attacker tries to make $7$'s predicted as $1$'s for EMNIST and horses as automobiles for CIFAR-10. The backdoor trigger is a $5$$\times$$5$-pixel black square at the bottom right corner of the image.
% An $\alpha$ fraction of the clients are chosen to be malicious, who are given $10$ corrupted samples. 
% We study first homogeneous and static settings, and we discuss   heterogeneous and dynamic settings in \S\ref{section:heterogeneous} and \S\ref{section:time_varying}. 


%\subsection{Experimental Results}

% \subsection{Backdoor Leakage}
% We consider a federated continual learning  where a model is trained for a long time and demonstrate how existing defenses all eventually fail. The reason is that even if a defense manages to reduce the effect of backdoor attacks in each round, a small fraction of gradients from the corrupted examples pass the filter, as no defense is perfect. This {\em backdoor leakage} eventually leads to a fully backdoored model as shown below. 
% %To show the backdoor leakage phenomenon in Fig. \ref{fig:backdoor_leakage},
% For a relatively small $\alpha=3\%$ and for $12,000$ rounds, we observe the attack success rate (ASR) of all competing  defenses eventually approach $1$.
% %Among all baselines, the representation-based SPECTRE has the slowest backdoor learning rate, and takes around $10000$ rounds to converge on ASR.
% On the other hand,  Algorithm~\ref{alg:framework} achieves an ASR of $0.0013$ for EMNIST and $0.0092$ for CIFAR-10.
% %The early stopped shadow network when the training accuracy on benign samples with the target label converges, ASR is independent of the training round.  %, indicating the success of the defense.
% These experiments are under the static setting where  data distribution is fixed over time; we show results in dynamic settings in \S~\ref{section:time_varying}. 


% \begin{figure}[htbp]
% \centering
% \subfigure[EMNIST dataset]{
% \includegraphics[width=0.46\linewidth]{img/003_longrun.pdf}
% }
% \subfigure[CIFAR-10 dataset]{
% \includegraphics[width=0.46\linewidth]{img/cifar_003.pdf}
% }
% \caption{Backdoor leakage causes competing defenses to fail eventually, even with a small $\alpha = 3\%$.\gf{We can move (b) to the appendix for space}}
% \label{fig:backdoor_leakage}
% \end{figure}


%Similar phenomenon appears in Fig. \ref{fig:backdoor_leakage}(b): ASR converges to around $0.95$ after $12000$ rounds in all baselines, while keeps as $0.0092$ in our algorithm.


\subsection{Defense under Homogeneous and Static Clients}
\label{section:homogeneous}


% For EMNIST, we also consider the homogeneous and manually-heterogeneous version by preprocessing the dataset.
In the homogeneous EMNIST dataset, we shuffle the dataset and 100 images are distributed  to each client. %before adding backdoor triggers. 
%  There are $\alpha$ fraction of clients who are adversarial and own extra $10$ corrupted images. 
We assume the target label $\ell=1$
 is known to the defender; we show what happens for unknown $\ell$ in Sec. \ref{app:unknown_label}. 
 We train the model for $1200$ rounds to model continuous training.
 Recall from Figure~\ref{fig:backdoor_leakage} that existing defenses  suffer from backdoor leakage when $\alpha$ is small ($\alpha=0.03$). 
 In contrast,  Algorithm~\ref{alg:framework} achieves an ASR of $0.0013$ for EMNIST and $0.0092$ for CIFAR-10.
%  and demonstrate how existing defenses all eventually fail. This is due to the backdoor leakage explained in Figure~\ref{fig:backdoor_leakage}. 
%Since the ASR in our algorithm is independent of the training round, we evaluate it after the shadow network being early-stopped. 
%The MTA of our algorithm is always larger than $0.995$ under homogeneous EMNIST, and is always between $92.5\%$ and $93.5\%$.
Algorithm \ref{alg:framework} also offers strong protection at higher $\alpha$.
For $\alpha$ as high as 0.45, Table~\ref{table:homo_EMNIST} shows that Algorithm~\ref{alg:framework} has an ASR below 0.06 and MTA above $0.995$ on EMNIST, whereas existing defenses all suffer from backdoor leakage. 
% The Main Task Accuracy (MTA) of Algorithm~\ref{alg:framework}  is always larger than $0.995$. 


%In this section, we evaluate the performance of our algorithm, and compare it with baseline defense algorithms with different malicious rate $\alpha\in[0.15, 0.45]$ under the homogeneous EMNIST and CIFAR-10 in Table \ref{table:homo_EMNIST} and \ref{table:cifar10}. For all baselines, we evaluate the ASR after the network being trained for $1200$ rounds. 


\begin{table}[htbp]
\caption{ASR for EMNIST under continuous training shows the advantage of Algorithm~\ref{alg:framework}, while others suffer  backdoor leakage.}
\label{table:homo_EMNIST}
\footnotesize
\centering
\vspace{4mm}
\begin{tabular}{ccccc}
\toprule
Defense $\setminus$
$\alpha$ & 0.15 & 0.25 & 0.35 & 0.45
%\(\alpha\) & \makecell[c]{Noise\\Adding} & \makecell[c]{Clipping and\\ Noise Adding} & RFA & \makecell[c]{G-SPECTRE} & \makecell[c]{R-SPECTRE} & \makecell[c]{Shadow Learning (Ours)\\ (label-level/user-level)} 
\\\midrule
Noise Adding & 1.00 & 1.00 & 1.00 & 1.00\vspace{0.8mm}\\
\vspace{0.8mm}
\makecell[c]{Clipping and\\ Noise Adding} & 1.00 & 1.00 & 1.00 & 1.00\\
RFA & 1.00 & 1.00 & 1.00 & 1.00\\
Multi-Krum & 1.00 & 1.00 & 1.00 & 1.00\\
FoolsGold & 0.9972 & 1.00 & 1.00 & 1.00\\
FLAME & 1.00 & 1.00 & 1.00 & 1.00\\
CRFL & 0.9873 & 0.9892 & 0.9903 & 0.9884\\
G-SPECTRE & 0.9948 & 1.00 & 1.00 & 1.00\\
R-SPECTRE & 0.9899 & 0.9934 & 1.00 & 1.00
\vspace{0.8mm}\\
\makecell[c]{Shadow Learning\\ %(Ours)\\
(label-level /\\ user-level)} & \makecell[c]{\textbf{0.0067}\ / \\ 0.0216} & \makecell[c]{\textbf{0.0101}\ /\\ 0.0367} & \makecell[c]{\textbf{0.0312}\ /\\ 0.0769} & \makecell[c]{\textbf{0.0502}\ /\\ 0.1338}\\
\bottomrule
\end{tabular}
\end{table}

In some scenarios, it might be infeasible to get access to average representations for the target label. In this case,  we propose a user-level defense whose ASR is also shown in the bottom row. We observe that ASR degrades gracefully, when switching to the user-level defense,  
%Under homogeneous EMNIST dataset, we also evaluate our method with user-level defense,
a variant of our algorithm in which each user uploads the averaged representation over all samples rather than samples with the target label. Data homogeneity enables Algorithm \ref{alg:framework} to distinguish malicious clients only based on averaged representations over all samples, without knowing the target label.
% Therefore, our algorithm does not require the knowledge of the target label under homogeneous dataset.
We experiment with heterogeneous clients in Section~\ref{section:heterogeneous}. 

%We can observe from Table \ref{table:homo_EMNIST} that the ASR of our algorithm is the lowest, and is only around $0.05$ when $\alpha = 0.45$. Our method with user-level defense also has low ASR, which is smaller than $0.08$ when $\alpha\leq 0.35$. The homogeneity enables our algorithm to distinguish malicious clients only based on averaged representations over all samples. Therefore, our algorithm does not require the knowledge of the target label under homogeneous dataset. For all baselines, the ASRs are always around $1.0$, which indicates the failure of them under federated continual learning settings.

\begin{table}[htbp]
\caption{ASR for CIFAR-10 under continuous training %changing data distribution 
shows the advantage of Algorithm~\ref{alg:framework}, while others suffer  backdoor leakage.}
\label{table:cifar10}
\footnotesize
\centering
\vspace{4mm}
\begin{tabular}{ccccc}
\toprule
Defense $\setminus$
$\alpha$ & 0.15 & 0.25 & 0.35 & 0.45
%\(\alpha\) & \makecell[c]{Noise\\Adding} & \makecell[c]{Clipping and\\ Noise Adding} & RFA & \makecell[c]{G-SPECTRE} & \makecell[c]{R-SPECTRE} & \makecell[c]{Shadow Learning (Ours)\\ (label-level/user-level)} 
\\\midrule
Noise Adding & 0.9212 & 0.9177 & 0.9388 & 0.9207
\vspace{0.8mm}\\
\vspace{0.8mm}
\makecell[c]{Clipping and\\ Noise Adding} & 0.9142 & 0.9247 & 0.9282 & 0.9338\\
RFA & 0.9353 & 0.9528 & 0.9563 & 0.9598\\
Multi-Krum & 0.9254 & 0.9196 & 0.9219 & 0.9301\\
FoolsGold & 0.8969 & 0.9038 & 0.9157 & 0.9143\\
FLAME & 0.9328 & 0.9267 & 0.9291 & 0.9331\\
CRFL & 0.8844 & 0.8731 & 0.8903 & 0.8891\\
G-SPECTRE & 0.8754 & 0.9001 & 0.9142 & 0.9193\\
R-SPECTRE & 0.7575 & 0.8826 & 0.8932 & 0.9091
\vspace{0.8mm}\\
\makecell[c]{Shadow Learning%\\ (Ours)
} & \makecell[c]{\textbf{0.0140}} & \makecell[c]{\textbf{0.0355}} & \makecell[c]{\textbf{0.0972}} & \makecell[c]{\textbf{0.1865}}\\
\bottomrule
\end{tabular}
\end{table}



Compared to EMNIST, CIFAR-10 is more difficult to learn. The smaller learning rate results in less effective early stopping  and thus leads to slightly larger ASR in Table \ref{table:cifar10}. %However, the ASR of our algorithm is still smaller than $0.04$ when $\alpha \leq 0.25$ and smaller than $0.19$ when $\alpha \leq 0.25$. The ASRs of all baselines are larger than $0.87$ in most cases, indicting the failure of them.
We show the ASR for CIFAR-100 and Tiny-ImageNet in Appendix \ref{app:homo_more}.






%To show that our backbone-shadow network framework has the best MTA-ASR tradeoff, we compare it with SPECTRE with representation version and RFA.
%We set the malicious rate as $15\%$ and $45\%$, and consider the static setting under .



%As in Fig.\ref{fig:tradeoff}, the green curve represents our algorithm, while the green star is the MTA-ASR point we achieve after adopting the proposed early-stopping mechanism.For both settings, our algorithm has the best MTA-ASR tradeoff, and achieves (0.9973, 0.0067) and (0.9967, 0.0502) MTA-ASR point respectively.
%When $\alpha = 15\%$, although representation-based SPECTRE has better MTA-ASR tradeoff among baselines, the MTA is smaller than $0.98$ when ASR is lower than $0.03$.
%When $\alpha = 45\%$, the MTA-ASR tradeoff of RFA is similar to that without defense method, and SPECTRE also has worse tradeoff, indicating these baselines cannot achieve the defense goal even combined with the early-stopping mechanism. 


\subsection{Ablation study under distribution drift}
\label{section:time_varying}

We next provide an ablation study to illustrate why the components of shadow learning are all necessary. 
We run this evaluation under a distribution drift scenario,
where the distribution changes every $400$ rounds. 
We use homogeneous EMNIST in the first phase $e_1$, then reduce the number of samples with labels $2$-$5$ to $10\%$ of the original  in phase $e_2$, %to $10\%$ of the original in phase $e_2$, 
i.e., we reduce the number of images with the label in $\{2, 3, 4, 5\}$ from $10$ to $1$ for each client. 
% In the third phase $e_
% 3$, we reduce the number of samples with labels $0$ and $1$ to $10\%$ of the original while keeping other samples as the same level in $e_1$, i.e., each client has one image for label $0$ and $1$ respectively, and ten images for any other label. 
Again, the backdoor target label is $1$. % it is reasonable (?) to
%We demonstrate
% Under EMNIST dataset in the dynamic setting, i.e.,  the data distribution changes over time, 


\begin{figure}
%\begin{wrapfigure}{L}{0.45\textwidth}
\vspace{-0.3cm}
\centering
% \subfigure[Phase $e_2$]{
\includegraphics[width=\linewidth]{img/015_2_2.pdf}
% }
% \subfigure[Phase $e_3$]{
% \includegraphics[width=0.4\linewidth]{img/015_earlystop_3.pdf}
% }
\caption{Ablation study for shadow learning under distribution drift. Simplified variants of our framework (e.g., periodic R-SPECTRE, shadow network prediction) significantly degrade the MTA-ASR Tradeoff with $\alpha = 0.15$, as achieving top-left is ideal. 
% after distribution shift (phase $e_2$) shows  is still close-to-ideal, despite the dynamic shift in clients' data.
}
\label{fig:time_varying}
\vspace{-0.15cm}
%\end{wrapfigure}
\end{figure}

We compare shadow learning with two simpler variants: Periodic R-SPECTRE and Shadow Network Prediction. 
In periodic R-SPECTRE, the backbone $N$ is retrained from scratch with SPECTRE every $R=400$ rounds; filtering is done in every round.
% is the interval of change in the client data. 
In Shadow Network Prediction, we use the same training as our framework, but prediction only uses the shadow network (as opposed to using the backbone network as in Algorithm~\ref{alg:framework}). 
%  assume that each malicious client contains one backdoor image.
The MTA-ASR tradeoffs of all three algorithms in the second phase  $e_2$ are shown in Fig.~\ref{fig:time_varying}.
Results for different periods and types of data distribution drift are shown in Appendix \ref{app:dynamic}.




%At the beginning of phase $e_2$, our algorithm detects the distribution change and renews the retraining process. 
Fig.\ref{fig:time_varying} shows that for $\alpha=0.15$, 
full shadow learning achieves an MTA-ASR point of $(0.9972, 0.0103)$ (green star),
% , adopting the early-stopping mechanism, Algorithm~\ref{alg:framework} achieves 
%and $(0.9903, 0.0234)$  
% in $e_2$. % and $e_3$, respectively. 
but the simplified variants perform significantly worse. 
% suffer from  the lack of training samples
% with labels $2$-$5$. % in phase $e_2$. 
%However, this distribution change has little effect on the how fast we learn images with the target  label $1$, and therefore our algorithm can achieve near-optimal tradeoff.
% The backbone network in Algorithm~\ref{alg:framework} persists throughout the training, and is thus resilient to data distribution changes; it achieves the green star point. 
% Fig.\ref{fig:time_varying}(b) shows that even when the proportion of samples with target label $\targetlabel=1$ sharply reduces, our algorithm can still achieve the defense goal. We provide more experiments in Appendix~\ref{app:dynamic}.  
Shadow network prediction does better than periodic R-SPECTRE, as it conducts client filtering only after the convergence of backbone network $\backbone$ on label $\targetlabel$,
while the latter filters in every round.
This indicates that filtering after $\backbone$ converges gives better  performance.
However, shadow network prediction suffers from the lack of training samples with labels $2$-$5$, leading to poor performance.
%In epoch $e_3$, the MTA is smaller than $0.97$ for our method with shadow Network prediction and smaller than $0.96$ for periodical representations-based SPECTRE when ASR is smaller than $0.03$.


\begin{table}[htbp]
\caption{ASR under EMNIST partitioned as the original data}
\label{table:EMNIST}
\centering
\vspace{4mm}
\small
\begin{tabular}{ccccc}
\toprule
Defense $\setminus$
$\alpha$ & 0.15 & 0.25 & 0.35 & 0.45
%\(\alpha\) & \makecell[c]{Noise\\Adding} & \makecell[c]{Clipping and\\ Noise Adding} & RFA & \makecell[c]{G-SPECTRE} & \makecell[c]{R-SPECTRE} & \makecell[c]{Shadow Learning (Ours)\\ (label-level/user-level)} 
\\\midrule
\makecell[c]{Label-level RFA} & 1.00 & 1.00 & 1.00 & 1.00\\
\makecell[c]{R-SPECTRE} & 0.9967 & 1.00 & 1.00 & 1.00
\vspace{0.8mm}\\
\vspace{0.8mm}
\makecell[c]{Shadow Learning\\ (Sample-level)} & \textbf{0.0107} & \textbf{0.0166} & \textbf{0.0301} & \textbf{0.0534}\\
Shadow Learning & 0.0307 & 0.0378 & 0.0836 & 0.1106
\vspace{0.8mm}\\
\vspace{0.8mm}
\makecell[c]{Shadow Learning\\ (User-level)} & 0.5719 & 0.5912 & 0.6755 & 0.7359\\
\bottomrule
\end{tabular}
\end{table}

\subsection{Defense without knowing target label $\ell$}
\label{app:unknown_label}

We next evaluate shadow learning when the defender only knows that the target label falls into a target set $S_\targetlabel$ on EMNIST.
In our generalized framework (Algorithm \ref{alg:framework_extend}), we set the training round threshold as $R=50$, and set the filtering ratio as $\kappa = 0.2$.
To analyze the averaged ASR and target label detection success rate, we set $\alpha = 0.3$ and vary the size of $S_\targetlabel$ from $2$ to $10$ (i.e., at $10$, the defender knows nothing about $\ell$). 
For each experimental setting, we run our framework $20$ times. 
% We also analyze the averaged QUE-ratio $\overline{\gamma}$ for each label when $|S_\targetlabel| = 10$.

\begin{figure}[htbp]
\centering
% \subfigure[Phase $e_2$]{
% \includegraphics[width=0.4\linewidth]{img/015_2_2.pdf}
% }
% \subfigure[Phase $e_3$]{
\includegraphics[width=0.85\linewidth]{img/adaptive_target_label.pdf}
% }
\caption{Defense Without Knowing the Exact Target Label with $\alpha = 0.3$}
\label{fig:adaptive_target_label}
\end{figure}


%\begin{figure}[htbp]
%\centering
%\subfigure[Averaged ASR and Target Label Detection Success Rate]{
%\includegraphics[width=0.47\linewidth]{img/adaptive_target_label.pdf}
%\label{fig:adaptive_target_label_asr}
%}
%\subfigure[Averaged QUE-ratio $\overline{\gamma}$ of Each Label]{
%\includegraphics[width=0.4\linewidth]{img/adaptive_target_label_gamma.pdf}
%\label{fig:adaptive_target_label_que}
%}
%\caption{Defense Without Knowing the Exact Target Label with $\alpha = 0.3$}
%\label{fig:adaptive_target_label}
%\end{figure}

As observed in Figure \ref{fig:adaptive_target_label}, when $|S_\targetlabel|\leq 9$, the averaged ASR of our method is near $0$, and the target label can be detected successfully all the time, i.e., target label $\targetlabel$ is in the filter target set $S'_{\targetlabel}$. When $|S_\targetlabel|= 10$, i.e., when the defender has no information about the target label, the averaged ASR and the detection success rates degrade gracefully (notice the different scales for the two vertical axes on Figure \ref{fig:adaptive_target_label}).
%Figure \ref{fig:adaptive_target_label_que} indicates that the averaged QUE-ratio of the target label ($>80$) is much larger than that of any other labels ($\approx 20$), which ensures the success of the target set filtering process in our framework.
This shows that \textbf{even without knowledge of the target label, shadow learning is still effective}. 

\subsection{Defense under Client Heterogeneity}
\label{section:heterogeneous}


We finally evaluate the ASR of Algorithm~\ref{alg:framework} and its two variants:  sample-level and user-level defenses. 
%under EMNIST and manually-heterogeneous EMNIST in Table \ref{table:EMNIST} and \ref{table:hetero_EMNIST} respectively.
In the sample level version, each user uploads the representations of samples with the target label without averaging, and the samples regarded as backdoor images are filtered out. This weakens privacy but is more robust against heterogeneous clients as shown in Table~\ref{table:EMNIST}. On the other hand, user-level defense fails as heterogeneity of clients makes it challenging to detect corrupt users from user-level aggregate statistics.
The label-level RFA and R-SPECTRE  are evaluated after the network is  trained for $1200$ rounds. More experimental results are provided in Appendix~\ref{app:hetero}.

\subsection{Other settings}
More experimental results including other datasets, defending against adaptive attack strategies (\ref{app:adaptive_alpha} and \ref{sec:fl_attack}), different trigger designs (\ref{sec:trigger}), and robustness to differentially-private noise \ref{sec:noise}, are shown in Appendix~\ref{sec:additional_exp}.

%Due to the heterogeneity of the dataset, the adversarial clients cannot be distinguished just based on the averaged representations over all local samples, and therefore the user level version of our algorithm fails to defense against the attacks.

%We also compare the performance of our algorithm with representation-based SPECTRE and label-level RFA in Table \ref{table:EMNIST}, where the ASRs of both comparing algorithms are evaluated after the network being trained for $1200$ rounds. For each label, the clients upload the aggregated gradients and then the  geometric median is estimated in label-level RFA. The server updates the model based on the average of these geometric medians.







%We can observe that the ASR of our algorithm is smaller than or equal to $0.04$ when $\alpha\leq 0.25$ and smaller than or equal to $0.13$ when $\alpha\leq 0.45$ for both EMNIST and manually-heterogeneous EMNIST.

%Instead of filtering out users, the sample level version of our algorithm filters out samples, which is more fine-grained, and thus has slightly smaller ASR. However, the central server cannot get access to the information of individual samples in the federated learning due to privacy issues, and our algorithm is an ideal replacement.


%We can also observe in Table \ref{table:EMNIST} that the ASRs of both comparing algorithms are $1$ in most cases, indicating the failure on achieving the defense goal.








